Scalable Topical Phrase Mining from Text Corpora

While most topic modeling algorithms model text corpora with unigrams, human interpretation often relies on inherent grouping of terms into phrases. As such, we consider the problem of discovering topical phrases of mixed lengths. Existing work either performs post processing to the inference results of unigram-based topic models, or utilizes complex n-gram-discovery topic models. These methods generally produce low-quality topical phrases or suffer from poor scalability on even moderately-sized datasets. We propose a different approach that is both computationally efficient and effective. Our solution combines a novel phrase mining framework to segment a document into single and multi-word phrases, and a new topic model that operates on the induced document partition. Our approach discovers high quality topical phrases with negligible extra cost to the bag-of-words topic model in a variety of datasets including research publication titles, abstracts, reviews, and news articles.

==> style/macro_2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Various theorem environments. All of the
% following have the same numbering system
% as theorem.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\reminder}[1]{[[ \marginpar[$=>$]{\flushleft$<=$}#1 ]]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Utilities
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%This command creates a box marked ``To Do'' around text.
%To use type \todo{  insert text here  }.

\newcommand{\todo}[1]{\vspace{5 mm}\par \noindent
 \marginpar{\textsc{ToDo}}
 \framebox{\begin{minipage}[c]{0.95 \textwidth}
 \tt #1 \end{minipage}}\vspace{5 mm}\par}

\newcommand{\eat}[1]{}

\def\papernumber #1 raised #2 {
  \vspace{-#2}
  \vbox to 0pt{\framebox{\bf Paper Number: #1}}
  %\vspace{#2}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Notions


% Spaces
\newcommand{\SEPR}{\hspace*{0.6cm}}
\newcommand{\sepr}{\hspace*{0.4cm}}
\newcommand{\smsep}{\hspace*{0.2cm}}
\newcommand{\s}{\hspace*{2mm}}
\newcommand{\noparag}{\hspace*{-\parindent}}
\newcommand{\parag}{\hspace*{ \parindent}}
\newcommand{\smgap}{-5pt}

% font styles
\newcommand{\un}{\underline}
\newcommand{\pf}{\sf}                   % Program font
\newcommand{\fs}{\small}                % Program font
\newcommand{\schf}{\footnotesize\tt}    % schema font
\newcommand{\PFB}[1]{\mbox{\pf \footnotesize #1}}
\newcommand{\PFBs}[1]{\mbox{\pf \scriptsize #1}}
\renewcommand{\ttdefault}{pcr}

% Type keywords
\newcommand{\SetOf}{\PFB{{SetOf}}}
\newcommand{\Rcd}{\PFB{{Rcd}}}
\newcommand{\Choice}{\PFB{{Choice}}}
\newcommand{\Str}{\PFB{{str}}}
\newcommand{\Int}{\PFB{{int}}}
\newcommand{\Flt}{\PFB{{float}}}

% Query keywords
\newcommand{\Set}{\PFB{\un{set}}}
\newcommand{\Let}{\PFB{\un{let}}}
\newcommand{\mf}{\PFB{\un{MF}}}
\newcommand{\mr}{\PFB{\un{MR}}}
\newcommand{\In}{~\PFB{\un{in}}~}
\newcommand{\Where}{\PFB{\un{where}}}
\newcommand{\With}{\PFB{\un{with}}}
\newcommand{\Select}{\PFB{\un{select}}}
%\newcommand{\For}{\PFB{\un{for}}}
\newcommand{\Orderby}{\PFB{\un{order by}}}
\newcommand{\Groupby}{\PFB{\un{group by}}}
\newcommand{\Limit}{\PFB{\un{limit}}}
%\newcommand{\Return}{\PFB{\un{return}}}
\newcommand{\From}{\PFB{\un{from}}}
\newcommand{\EAnd}{~\PFB{\un{and}}~}
\newcommand{\Tuple}{\PFB{~\un{struct}~}}
\newcommand{\Exists}{\PFB{\un{exists}}}
\newcommand{\Element}{\PFB{~\un{element}~}}
\newcommand{\Foreach}{\PFB{\un{foreach}}}
\newcommand{\Every}{\PFB{\un{every}}}
%\newcommand{\If}{\PFB{\un{if}}}
\newcommand{\Then}{\PFB{\un{then}}}
\newcommand{\Satisfies}{\PFB{\un{satisfies}}}
%\newcommand{\SetID}{\PFB{SetID}}
%\newcommand{\Null}{~\PFB{~\un{null}~}}
%\newcommand{\Construct}{~\PFB{~\un{construct}~}}

\newcommand{\Ins}{~\PFBs{\un{in}}~}
\newcommand{\Wheres}{\PFBs{\un{where}}}
\newcommand{\Withs}{\PFBs{\un{with}}}
\newcommand{\Selects}{\PFBs{\un{select}}}
\newcommand{\Fors}{\PFBs{\un{for}}}
\newcommand{\Returns}{\PFBs{\un{return}}}
\newcommand{\Froms}{\PFBs{\un{from}}}
\newcommand{\EAnds}{~\PFBs{\un{and}}~}
\newcommand{\Tuples}{\PFBs{~\un{struct}~}}
\newcommand{\Existss}{\PFBs{\un{exists}}}
\newcommand{\Elements}{\PFBs{~\un{element}~}}
\newcommand{\Foreachs}{\PFBs{\un{foreach}}}
\newcommand{\Everys}{\PFBs{\un{every}}}
\newcommand{\Ifs}{\PFBs{\un{if}}}
\newcommand{\Thens}{\PFBs{\un{then}}}
\newcommand{\Satisfiess}{\PFBs{\un{satisfies}}}
\newcommand{\expl}{\mbox {\tt Expl}}
\newcommand{\itemsim}{\mbox {\tt ItemSim}}
\newcommand{\usersim}{\mbox {\tt UserSim}}
\newcommand{\calu}{\mbox {$\cal U$}}
\newcommand{\cali}{\mbox {$\cal I$}}
\newcommand{\nw}{\mbox {\tt Network}}
\newcommand{\ddu}{\mbox {$DD_u$}}
\newcommand{\ddju}{\mbox {$DD^J_u$}}
\newcommand{\ddcu}{\mbox {$DD^C_u$}}
\newcommand{\socrel}{\mbox {\tt SocRel}}

\newcommand{\from}[2]{{\sc from} {\bf #1: #2}}

\newcommand{\ch}{$\rightarrow$}
\newcommand{\mt}[1]{$#1$}
\newcommand{\mc}[1]{$\mathcal{#1}$}
\newcommand{\mcs}[2]{$\mathcal{#1}_{#2}$}
\newcommand{\tbd}{\textbf{TBD}}

\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}
\newtheorem{example}{Example}
%\newtheorem{fd}{FD}
\newtheorem{property}{Property}
\newtheorem{principle}{Principle}

\newtheorem{Ob}{Observation}

\newenvironment{query}{
\footnotesize
\vspace*{\smgap}
\begin{tabbing} }
{\end{tabbing}
\normalsize\small\normalsize
\vspace*{\smgap}
}

\newenvironment{querys}{
\scriptsize
\vspace*{\smgap}
\begin{tabbing} }
{\end{tabbing}
\normalsize\small\normalsize
\vspace*{\smgap}
}

% Bolin
\newcommand{\cequ}{Equation~}
\newcommand{\cequs}{Equations~}
\newcommand{\csec}{Section~}
\newcommand{\csecs}{Sections~}
\newcommand{\cexa}{Example~}
\newcommand{\cdef}{Definition~}
\newcommand{\cthm}{Theorem~}
\newcommand{\cthms}{Theorems~}
\newcommand{\clem}{Lemma~}
\newcommand{\clems}{Lemmas~}
\newcommand{\calg}{Algorithm~}
\newcommand{\cfig}{Figure~}
\newcommand{\db}{{\cal D}\xspace}
\newcommand{\col}{{\rm col}\xspace}
\newcommand{\ie}{i.e.\xspace}
\newcommand{\eg}{e.g.\xspace}
\newcommand{\ind}{^{\rm th}\xspace}
\newcommand{\schemaG}{{\cal G}\xspace}
\newcommand{\schemaV}{{\cal V}\xspace}
\newcommand{\schemaE}{{\cal E}\xspace}
\newcommand{\joinG}{{\cal J}\xspace}
\newcommand{\projectC}{{\cal C}\xspace}
\newcommand{\mapping}{{\phi}\xspace}
\newcommand{\answer}{{\cal A}\xspace}
\newcommand{\stitle}[1]{\vspace{1ex} \noindent{\bf #1}}
\newcommand{\candq}{{\cal Q}\xspace}
\newcommand{\cand}{{\cal Q_{\rm C}}\xspace}
\newcommand{\candu}{{\cal Q_{\rm X}}\xspace}
\newcommand{\candp}{{\cal Q_{+}}\xspace}
\newcommand{\candn}{{\cal Q_{-}}\xspace}
\newcommand{\filter}{{\cal F}\xspace}
\newcommand{\filteru}{{\cal F}_{\rm X}\xspace}
\newcommand{\filterB}{{\cal F}_{\rm B}\xspace}
\newcommand{\opt}{{\rm OPT}\xspace}
\newcommand{\sol}{{\rm SOL}\xspace}
\newcommand{\cost}{{\rm cost}\xspace}
\newcommand{\minimum}{{\rm MIN}\xspace}
\newcommand{\basic}{{\rm BAS}\xspace}
\newcommand{\bigoh}{{\rm O}\xspace}
\newcommand{\dependT}{\succ_+\xspace}
\newcommand{\dependF}{\succ_-\xspace}
\newcommand{\eval}{{\rm ex}\xspace}
\newcommand{\pr}[1]{{\bf Pr}\left[#1\right]\xspace}
\newcommand{\ep}[1]{{\bf E}\left[#1\right]\xspace}
\newcommand{\workload}{{\rm W}\xspace}

\newtheorem{corr}{Corollary}
\newtheorem{lemma}{Lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   End
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

